Efficient Methods for Approximating the Shapley Value for Asset Sharing in Energy Communities

With the emergence of energy communities, where a number of prosumers invest in shared generation and storage, the issue of fair allocation of benefits is increasingly important. The Shapley value has attracted increasing interest for redistribution in energy settings - however, computing it exactly is intractable beyond a few dozen prosumers. In this paper, we first conduct a systematic review of the literature on the use of Shapley value in energy-related applications, as well as efforts to compute or approximate it. Next, we formalise the main methods for approximating the Shapley value in community energy settings, and propose a new one, which we call the stratified expected value approximation. To compare the performance of these methods, we design a novel method for exact Shapley value computation, which can be applied to communities of up to several hundred agents by clustering the prosumers into a smaller number of demand profiles. We perform a large-scale experimental comparison of the proposed methods, for communities of up to 200 prosumers, using large-scale, publicly available data from two large-scale energy trials in the UK (UKERC Energy Data Centre, 2017, UK Power Networks Innovation, 2021). Our analysis shows that, as the number of agents in the community increases, the relative difference to the exact Shapley value converges to under 1% for all the approximation methods considered. In particular, for most experimental scenarios, we show that there is no statistical difference between the newly proposed stratified expected value method and the existing state-of-the-art method that uses adaptive sampling (O'Brien et al., 2015), although the cost of computation for large communities is an order of magnitude lower.

==> pseudocodes/shapley_RL.tex <==
\begin{algorithm*}[!tbp]
  \caption{Cost redistributed to agent $i$ according to the reinforcement learning Shapley Approximation method~\cite{7101858}}
  \label{alg:shapley_RL}
  \begin{algorithmic}[1]
  \Require{Set of prosumers in the community, $\mathcal{N}$, with a size of $N$. Agent $i$ in the community. Number of samples drawn per agent, $M$.} 
  \Ensure {The redistributed energy costs of agent $i$, $bill_i$.}
  \Statex
    \Function{ApproximateShapleyRL}{$\mathcal{N}, i, M$}
        \State $\hat \mu_{i,j} \gets 0, \; j = 0,...,N-1$ \Comment{Estimated mean marginal contribution of agent $i$ at stratum $j$}
        \State $\hat \sigma_{i,j} \gets 10000, \; j = 0,...,N-1$ \Comment{Estimated SD of marginal contribution of agent $i$ at stratum $j$}
        \State $h_{i,j} \gets 0, \; j = 0,...,N-1$\Comment{Count of how many times it was sampled from stratum $j$}
        \State $m2_{i,j} \gets 0, \; j = 0,...,N-1$\Comment{Sum of squared differences from the mean of stratum $j$}
        \For{$m \gets 1$ to $M$}
            \State $\pi_{i,j}(m) = \frac{\epsilon(m)}{N} + (1 - \epsilon(m))\frac{\hat \sigma_{i,j}}{\sum_{s=0}^{N-1} \hat \sigma_{i,s}}, \; j = 0,...,N-1$ \Comment{Probability of $i$ selecting stratum $j$ at sample $m$, $\epsilon(m)$ from Eq.~\ref{eq:epsilon}}
            \State choose stratum $j$ where $0 \leq j \leq N-1$ according to probabilities $\pi_{i}(m)$
            \State choose a random coalition $\mathcal{S} \subseteq \mathcal{N} \setminus \{i\}$ where $\lvert \mathcal{S} \rvert = j$
            
            \State $h_{i,j} \gets h_{i,j} + 1$ \Comment{Update count of stratum $j$}
            \State $mc \gets c(\mathcal{S}\cup\{i\}) - c(\mathcal{S})$\Comment{Marginal contribution}
            \State $\Delta \gets mc - \hat \mu_{i,j}$
            \State $\hat \mu_{i,j} \gets \hat \mu_{i,j} + \frac{\Delta}{h_{i,j}}$\Comment{Update estimated marginal contribution of stratum $j$}
            \State $m2_{i,j} \gets m2_{i,j} + \Delta (mc - \hat \mu_{i,j})$
            \If{$h_{i,j} > 1$}
                \State $\hat \sigma_{i,j} \gets \sqrt{\frac{\hat \sigma_{i,j}}{h_{i,j} - 1}}$ \Comment{Update estimated SD of stratum $j$ if it is sampled more than once}
            \EndIf
        \EndFor
        \State $bill_i \gets \frac{1}{N}\sum_{j=0}^{N-1} \hat  \mu_{i,j}$\Comment{Mean of all strata for agent $i$, equivalent to $b^{rl}_i$}

        \State \textbf{return} $bill_i$
    \EndFunction
  \end{algorithmic}
\end{algorithm*}
